Conformal k-NN Anomaly Detector for Univariate Data Streams

Anomalies in time-series data give essential and often actionable information in many applications. In this paper we consider a model-free anomaly detection method for univariate time-series which adapts to non-stationarity in the data stream and provides probabilistic abnormality scores based on the conformal prediction paradigm. Despite its simplicity the method performs on par with complex prediction-based models on the Numenta Anomaly Detection benchmark and the Yahoo! S5 dataset.

==> yahoo_results.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  reward\_low\_FN\_rate &  reward\_low\_FP\_rate &  standard \\
\midrule
bayesChangePt    &                43.6 &                17.6 &      35.7 \\
knn              &                68.2 &                56.6 &      63.5 \\
knn1             &                50.0 &                 0.1 &      36.0 \\
knn2             &                50.0 &                 0.1 &      36.0 \\
knn3             &                68.2 &                56.6 &      63.5 \\
knn4             &                68.2 &                56.4 &      63.8 \\
knn5             &                50.0 &                 0.3 &      36.1 \\
knncad           &                68.8 &                57.0 &      64.3 \\
knncad1          &                50.0 &                 0.1 &      36.0 \\
knncad2          &                50.0 &                 0.1 &      36.0 \\
knncad3          &                68.8 &                57.0 &      64.3 \\
knncad4          &                68.8 &                56.9 &      64.3 \\
knncad5          &                50.1 &                 0.4 &      36.1 \\
knnoneone        &                51.4 &                36.4 &      46.0 \\
knnoneone1       &                43.6 &                18.0 &      36.2 \\
knnoneone2       &                30.7 &               -20.7 &      16.9 \\
knnoneone3       &                50.6 &                35.1 &      44.7 \\
knnoneone4       &                50.6 &                35.2 &      44.8 \\
knnoneone5       &                30.8 &               -20.7 &      16.9 \\
knnoneonecad     &                53.4 &                35.9 &      46.1 \\
knnoneonecad1    &                47.5 &                20.9 &      37.3 \\
knnoneonecad2    &                47.7 &                21.5 &      37.6 \\
knnoneonecad3    &                53.8 &                36.2 &      46.9 \\
knnoneonecad4    &                53.8 &                36.2 &      46.9 \\
knnoneonecad5    &                47.7 &                21.5 &      37.6 \\
null             &                 0.0 &                 0.0 &       0.0 \\
numenta          &                44.4 &                37.5 &      41.0 \\
numentaTM        &                42.5 &                36.6 &      39.4 \\
random           &                47.2 &                 1.2 &      29.9 \\
relativeEntropy  &                52.5 &                40.7 &      48.0 \\
skyline          &                28.9 &                18.0 &      23.6 \\
windowedGaussian &                40.7 &                25.8 &      31.1 \\
\bottomrule
\end{tabular}

